Unveiling new disease, pathway, and gene associations via multi-scale neural networks

Diseases involve complex processes and modifications to the cellular machinery. The gene expression profile of the affected cells contains characteristic patterns linked to a disease. Hence, biological knowledge pertaining to a disease can be derived from a patient cell's profile, improving our diagnosis ability, as well as our grasp of disease risks. This knowledge can be used for drug re-purposing, or by physicians to evaluate a patient's condition and co-morbidity risk. Here, we look at differential gene expression obtained from microarray technology for patients diagnosed with various diseases. Based on this data and cellular multi-scale organization, we aim to uncover disease--disease links, as well as disease-gene and disease--pathways associations. We propose neural networks with structures inspired by the multi-scale organization of a cell. We show that these models are able to correctly predict the diagnosis for the majority of the patients. Through the analysis of the trained models, we predict and validate disease-disease, disease-pathway, and disease-gene associations with comparisons to known interactions and literature search, proposing putative explanations for the novel predictions that come from our study.

==> neural_network.tex <==
\tikzstyle{state}=[circle,draw=black,fill=none,minimum size=20pt,inner sep=0pt]
		\tikzstyle{edge} = [draw,thick,-]
		\hspace{-5em}\begin{figure*}[ht]
			\centering
			\scalebox{0.9}{\begin{tikzpicture}[-,auto,node distance=1cm,thick]
				\node[state] (A) {};
				\node[state,draw=none, align=center]  (H) [above of = A] { \large Genes};
				\node[state] (B) [below of= A] {};
				\node[state] (C) [below of= B] {};
				\node[state] (D) [below of= C] {};
				\node[state] (E) [below of= D] {};
				\node[state] (F) [below of= E] {};
				\node[state] (G) [below of= F] {};
				
				
				\node[state,draw=none, node distance=1cm, align=center]  (H0) [left of = H] {};
				\node[state] (A0) [below of= H0] {};
				\node[state] (B0) [below of= A0] {};
				\node[state] (C0) [below of= B0] {};
				\node[state] (D0) [below of= C0] {};
				\node[state] (E0) [below of= D0] {};
				\node[state] (F0) [below of= E0] {};
				\node[state] (G0) [below of= F0] {};
				\node[state,rotate=90,draw=none,align = center, node distance =1cm] (input) [above of = D0] {\large Gene Expressions};
				
				\node[state,draw = none, node distance=4cm, align=center] (lbl2) [right of = H] {\large Biological\\\large Pathways};
				\node[state, node distance=2cm] (a2) [below of =lbl2] {};
				\node[state, node distance=1cm] (b2) [below of=a2] {};
				\node[state, node distance=1cm] (c2) [below of=b2] {};
				\node[state, node distance=1cm] (d2) [below of=c2] {};
				\node[state, node distance=1cm] (e2) [below of=d2] {};
				
				\node[state,draw = none, node distance=4cm, align=center] (lbl3) [right of = lbl2] {\large Phenotypes\\\large (Diseases)};
				\node[state, node distance=2.5cm] (a3) [below of =lbl3] {};
				\node[state, node distance=1cm] (b3) [below of=a3] {};
				\node[state, node distance=1cm] (c3) [below of=b3] {};
				\node[state, node distance=1cm] (d3) [below of=c3] {};
				
				
				% First layer
				\path (A0) edge [->] (A)
				(B0) edge [->] (B)
				(C0) edge [->] (C)
				(D0) edge [->] (D)
				(E0) edge [->] (E)
				(F0) edge [->] (F)
				(G0) edge [->] (G);
				
				
				% First layer
				\path (A) edge (a2)
				(A) edge (b2)
				(B) edge (b2)
				(C) edge (b2)
				(C) edge (c2)
				(D) edge (c2)
				(D) edge (d2)
				(E) edge (d2)
				(E) edge (e2)
				(F) edge (d2)
				(F) edge (e2)
				(G) edge (b2)
				(G) edge (e2);
				
				% Final layer
				\path (a2) edge (a3)
				(a2) edge (b3)
				(a2) edge (c3)
				(a2) edge (d3)
				(b2) edge (a3)
				(b2) edge (b3)
				(b2) edge (c3)
				(b2) edge (d3)
				(c2) edge (a3)
				(c2) edge (b3)
				(c2) edge (c3)
				(c2) edge (d3)
				(d2) edge (a3)
				(d2) edge (b3)
				(d2) edge (c3)
				(d2) edge (d3)
				(e2) edge (a3)
				(e2) edge (b3)
				(e2) edge (c3)
				(e2) edge (d3);
				
				\end{tikzpicture}}
				\caption{\label{fig:nn} Example of neural network architecture. For the first layer, the connections are defined by biological information, i.e. a unit representing a gene is connected to all the biological pathways that the gene is involved in. We do not add any prior knowledge on the last layer, thus it is fully connected.}
		\end{figure*}
	
